Semi-supervised learning for marine anomaly detection on board satellites

Aquatic bodies face numerous environmental threats caused by several marine anomalies. Marine debris can devastate habitats and endanger marine life through entanglement, while harmful algal blooms can produce toxins that negatively affect marine ecosystems. Additionally, ships may discharge oil or engage in illegal and overfishing activities, causing further harm. These marine anomalies can be identified by applying trained deep learning (DL) models on multispectral satellite imagery. Furthermore, the detection of other anomalies, such as clouds, could be beneficial in filtering out irrelevant images. However, DL models often require a large volume of labeled data for training, which can be both costly and time-consuming, particularly for marine anomaly detection where expert annotation is needed. A potential solution is the use of semi-supervised learning methods, which can also utilize unlabeled data. In this project, we implement and study the performance of FixMatch for Semantic Segmentation, a semi-supervised algorithm for semantic segmentation. Firstly, we found that semi-supervised models perform best with a high confidence threshold of 0.9 when there is a limited amount of labeled data. Secondly, we compare the performance of semi-supervised models with fully-supervised models under varying amounts of labeled data. Our findings suggest that semi-supervised models outperform fully-supervised models with limited labeled data, while fully-supervised models have a slightly better performance with larger volumes of labeled data. We propose two hypotheses to explain why fully-supervised models surpass semi-supervised ones when a high volume of labeled data is used. All of our experiments were conducted using a U-Net model architecture with a limited number of parameters to ensure compatibility with space-rated hardware.

==> 3_MethodsAblation_study_lr_decay.tex <==
\subsection{Ablation Study - Learning Rate Decay in Fully-Supervised Models}  \label{exp:lr-decay-fully-sup}


An important step is how to choose the fully-supervised baseline models whose performance (in terms of evaluation metrics) will be compared against the semi-supervised models. In \cite{kikaki2022marida}, the tested neural network was trained for 45 epochs with a learning rate equal to $2e\text{-}4$ and a learning rate decay that multiplied the learning rate by $0.1$ after the epoch number 40.  


We conduct an experiment to test if the performance of the fully-supervised baseline can be improved. In particular, an ablation study of the application of the learning rate decay at the \nth{40} epoch is performed. We decided to conduct the ablation study of this hyperparameter because decaying the learning rate too early could cause the model optimization to get stuck in a local minimum and therefore a worsening of the final performance.

The ablation study makes use of the same labeled training configurations presented in Subsubsection \ref{subsec:lab-train-config}. However, not all the percentages of the full training set are evaluated, primarily due to time limitations. Specifically, we opted to examine three percentages of labeled data representing low (10\%), medium (50\%), and high (80\%) percentages from the “Two Training Sets” configuration (refer to Subsection \ref{subsec:two-train-set}). This approach was chosen to avoid the necessity of testing every possible percentage of labeled data.

Given a percentage of labeled data, we will compare a pair of fully-supervised models. The first is trained with learning rate decay at the \nth{40} epoch, while the second is trained without learning rate decay. 
The same labeled subset ($\mathcal{D}^l$, refer to Subsection \ref{subsec:two-train-set}) is used to train a pair of fully-supervised models. The used evaluation method is the one described in Subsection \ref{subsec:exp-eval-metric}. %However, for this particular experiment, we opted to consider the minimum focal loss on the validation set as our performance metric, rather than the maximum mIoU on the same set. This was due to the fact that at the time of conducting this experiment, we had not yet begun logging the mIoU on the validation set.  





\subsubsection{Hyperparameters' Values}

The hyperparameters' values of the fully-supervised models are listed in Table \ref{table:hyperparams_fully-sup_comparison}. 

All hyperparameters are the same used in \cite{kikaki2022marida}, except for the number of epochs, and the alphas and gamma coefficients of the focal loss. We decided to train for more epochs (2000 instead of 45) to see if the performance could improve. The coefficients of the focal loss were added due to the fact that we decided to use the focal loss (refer to Subsection \ref{subsubsec:focal-loss}), which was not employed in \cite{kikaki2022marida}.


A comprehensive description of these hyperparameters can be found in Table \ref{table:hyperparams_descritption}.



\begin{table}[H]
\caption{Hyperparameters' values of the tested fully-supervised models.}
\label{table:hyperparams_fully-sup_comparison}
\centering
\begin{tabular}{ll}
    \toprule
    epochs                         & \multicolumn{1}{r}{2000}                             \\ 
    lr                         & \multicolumn{1}{r}{2e-4}                             \\ 
    batch size                 & \multicolumn{1}{r}{5}                                \\ 
    %\textbf{lr steps}  & 40                               \\ \hline
    alphas ($\alpha$)                    & \multicolumn{1}{r}{$\left[ 1, 1, 1, 1, 1\right]$} \\
    gamma ($\gamma$)                     & \multicolumn{1}{r}{2.0} \\ 
    \bottomrule                            
\end{tabular}
\end{table}

% fully-sup -> same hyperparams as the original work from kikkaki
% semi-sup -> random search to perform some hyperp-tuning

==> 3_MethodsOne_train_set_1.tex <==
\subsection{One Training Set Setting}
\label{subsec:one-train-set}

The "One Training Set" approach utilizes the complete original MARIDA training set as its sole training set.

Every image has labeled and unlabeled pixels. In the context of training, fully-supervised models utilize only the labeled pixels, while semi-supervised models use both labeled and unlabeled pixels.

In this scenario, all labeled pixels from every training image are utilized during the training process. This is in contrast to the "Two Training Sets" approach, which only employs the labeled pixels from images present in $\mathcal{D}^l$.

When training using the "One Training Set" setting, a training epoch is defined as one complete cycle of training the model using the entire training set. And each epoch consists of several training steps.

==> 3_MethodsOne_train_set_2.tex <==
\subsection{Fully- versus Semi-Supervised Learning Models with One Training Set}
\label{subsec:exp_design_exp_1_train_set}

This experiment is designed to assess the performance of fully-supervised and semi-supervised learning models within the “One Training Set” framework. The focus is on determining whether FixMatch for semantic segmentation can improve performance by leveraging all labeled pixels and additional unlabeled pixels. This is compared against fully-supervised models that utilize only labeled pixels.

In this scenario, fully-supervised models compute the loss only on the labeled pixels of each image, while ignoring the unlabeled ones. On the other hand, semi-supervised models compute the loss on both labeled and unlabeled pixels of each image. More precisely, semi-supervised models compute the supervised component ($\mathcal{L}^s$, see \ref{subsubsec:sup_loss}) of the loss only on labeled pixels and the unsupervised component ($\mathcal{L}^u$, see \ref{subsubsec:unsup_loss}) only on unlabeled pixels.


In both fully- and semi-supervised models, every labeled pixel of the full training dataset contributes to the computation of the supervised loss.


The used evaluation method is the one described in \ref{subsec:exp-eval-metric}.



\subsubsection{Hyperparameters' Values of Semi-Supervised Models - One Training Set}

The hyperparameters' values of the semi-supervised models tested in the "One Training Set" setting are listed in Table \ref{table:hyperparams_ssl_one_train_set}. The description of the hyperparameters is noted in Table \ref{table:hyperparams_descritption}. 

\begin{table}[H]
\centering
\begin{tabular}{l|l}
\hline
epoch                         & 2000                             \\ \hline
lr                         & 2e-4                             \\ \hline
batch size                 & 5                                \\ \hline
alphas ($\alpha$)                     & \left[1, 1, 1, 1, 1\right] \\ \hline
gamma ($\gamma$)                      & 2.0 \\ \hline 
threshold ($\tau$)                & 0.999                                \\ \hline
%reduce lr on plateau                 & 0                                \\ \hline
lambda coeff ($\lambda$)                 & 1                                \\ \hline

                           
\end{tabular}
\caption{Hyperparameters' values of the fully- and semi-supervised models tested in the "One Training Set" setting.}
\label{table:hyperparams_ssl_one_train_set}
\end{table}

==> 3_l1c_dataset.tex <==


\subsection{L1C Dataset}
\label{subsec:methods_l1c_dataset}



% description and motivation (add in the marida part which bands are there and the detail of the atmospheric correction. So you can motivate better l1c. Add a brief description of L1C bands when talking of Sentinel2? And write that Marida uses L1C but with atmosperic corr and without band 9 and 10.
In \cite{kikaki2022marida}, the images of the MARIDA dataset are post-processed with an atmospheric correction and they do not include bands B09 and B10. Applying the atmospheric correction is an operation that can be time-consuming to execute and is generally not performed onboard satellite hardware.

The idea is to create an L1C dataset \textit{(i)} that does not have an additional atmospheric correction pre-process step; \textit{(ii)} whose images correspond to the areas of the Earth's surface of the locations of the MARIDA dataset images; \textit{(iii)} that has also the bands B09 and B10. The name L1C comes from the Sentinel-2 Level-1C product (see \ref{subsec:product-levels-s2} for more details).


We construct this dataset to evaluate whether the deep-learning models we use will be able to perform on lower-level images as well as on higher-level images. This serves as a preliminary step in our research on the implementation of AI models onboard artificial satellites.

The correspondence of the L1C dataset patches to the MARIDA patches is necessary to be able to utilize the MARIDA dataset segmentation maps when training DL models.



\subsubsection{Image Retrieval}
\label{subsubsec:image-retr}
% Cop Hub image retrieval
% pyraws

The first task of the creation of the L1C dataset is to download all the L1C tiles containing the L1C patches that correspond to the areas of the Earth's surface of the MARIDA patches. A tile is an image that is composed of multiple patches.

The L1C tiles are downloaded from the Copernicus Open Access Hub \cite{cop_hub}%
. The following information are necessary to download a tile from the Copernicus Open Access Hub: the identifier of the tile, the date of the acquisition of the tile, the satellite that acquired the tile, and the product type. Since the MARIDA dataset is based on Sentinel-2 multispectral images, the satellite that acquired the data is Sentinel-2. The chosen product type is Level-1C, which on the Copernicus Open Access Hub is reported as \textit{S2MSI1C} (Sentinel-2 Multispectral Instrument L1C). Given a patch from the MARIDA dataset, the identifier and the date of acquisition of the tile can be easily retrieved. For instance, given the name of the MARIDA patch \textit{S2\_1-12-19\_48MYU\_0}, the identifier and the date of acquisition of the tile in which the patch is contained are respectively \textit{48MYU} and \textit{1-12-19}. The date of acquisition is in the format dd-mm-yy. The names of the patches of the MARIDA dataset are included in the training, validation and test split files. 

At this point, all L1C tiles can be obtained. However, as previously mentioned, an L1C patch is just a portion of the downloaded L1C tile in which it is contained. 

Thus, the following step consists in extracting, from each L1C tile, all the L1C patches that corresponds to the Earth’s surface location of the MARIDA patches. Firstly, the geo-referenced coordinates of the four corners of a MARIDA patch are extracted. Secondly, the retrieval of an L1C patch corresponding to a MARIDA patch is executed with PyRawS\footnote{https://github.com/ESA-PhiLab/PyRawS\label{footnote:pyraws}}, which is an open-source software providing utilities to open and process Sentinel-2 raw data. Thus, every L1C patch corresponding to a MARIDA patch is retrieved.


\subsubsection{Keypoint Matching}
% SuperGlue and keypoint matching

During the image retrieval phase (\ref{subsubsec:image-retr}), it was noticed that MARIDA patches and their corresponding L1C patches did not perfectly correspond. %
For example, one patch could cover a larger area of the Earth's surface than the other. It is important to note that the pixel-level correspondence with MARIDA patches is necessary since the ground-truth segmentation maps are based on MARIDA patches. And a misalignment of the segmentation maps with the patches could entirely compromise the learning of the network.

% add constant to all 4 sides
To overcome this problem, a larger area was considered when retrieving an L1C patch corresponding to a MARIDA patch with PyRawS\footref{footnote:pyraws}. The addition (or subtraction) of a constant to the geo-referenced coordinates of the four corners of a MARIDA patch enlarges the considered area covered by an L1C patch. Thus, the addition (or subtraction) makes sure that the L1C patch entirely contains the area of the Earth's surface of the correspondent MARIDA patch. 

So, at this stage, each L1C patch is a multispectral image that contains the same area acquired in the corresponding MARIDA patch, plus some additional pixels (corresponding to an extension of the area contained in the MARIDA patch) at the borders. Figure \ref{Figure:marida_l1c_after_constant} shows an example of a MARIDA patch and its corresponding L1C patch, which covers a larger area of the Earth's surface.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{images/3_Methods/L1C/after_adding_constant.pdf}
    \caption{Comparison of band B1 of a MARIDA patch and band B1 of its corresponding L1C patch covering a larger area of the Earth's surface.}
    \label{Figure:marida_l1c_after_constant}
\end{figure}


Having a larger L1C patch is not ideal since the segmentation maps corresponds to the MARIDA patch. Therefore, \textit{Superglue} \cite{sarlin2020superglue} was used to perform keypoint matching between the L1C and MARIDA patches. 
First, a CNN computes features from each of the two images. Then, Superglue tries to find the best-matching pairs between the two sets of features.

%Superglue is a  neural network that finds the matches among two sets of extracted features and assigns a score to them. A CNN computes the two set of features from two images. In this case, the two images are a pair of corresponding L1C and MARIDA patches.




However, every MARIDA and L1C patch is composed of multiple bands. For this reason, the matching keypoints are computed among each corresponding band of two corresponding L1C and MARIDA images. This computation is not applied to bands B09 and B10 because MARIDA patches do not include those.

%$\begin{figure}[H]
%    \centering
%    \begin{minipage}{0.45\textwidth}
%        \centering
%        \includegraphics[width=0.9\textwidth]{a} 
%        \caption{Example of }
%    \end{minipage}\hfill
%    \begin{minipage}{0.45\textwidth}
%        \centering
%        \includegraphics[width=0.9\textwidth]{b} 
%        \caption{second figure}
%    \end{minipage}
%    \caption{aaaa.}
%    \label{Figure:ahahgaoijai}
%\end{figure}


\subsubsection{Calculation of the correspondence}
% shift and crop

In this stage, the matching keypoints of a pair of corresponding L1C and MARIDA patches are already computed. Now, it is possible to estimate how to crop the larger L1C patch to make it match exactly the MARIDA patch. The two patches exactly match if the pixels of their corresponding bands represent the same Earth's surface area. The following paragraphs describe how the cropping procedure was performed by taking into consideration a single L1C patch and its corresponding MARIDA patch.

First of all, it is important to note that the segmentation map provided by the MARIDA dataset is the same for every band of a single MARIDA patch. Thus, every band of an L1C patch has to be cropped at the same location to make it match the corresponding MARIDA band. The steps that are applied to crop the larger L1C patch to match the corresponding MARIDA patch are the following: \first compute the mean of shifts of coordinates of matching keypoints, \second apply the mean shifts to the center's coordinates of the MARIDA patch, \third crop the larger L1C patch according to the original dimensions of the MARIDA patch.

Firstly, in step \first, the mean and standard deviation of both horizontal and vertical differences of coordinates of matching keypoints of all bands are computed. Figure \ref{Figure:shifts_example} shows an illustration of horizontal and vertical shifts of coordinates of matching keypoints. 

Then, all horizontal and vertical differences whose value is not in the interval $\left[ \mu - \sigma, \mu + \sigma \right]$ are discarded to remove outliers. Indeed, while checking the matching keypoints of some images, we found that the majority of them were correct but there were a minority of incorrect matches too. Incorrect matches can alter the averages that are going to be applied in step \second, and therefore detrimentally affect the correspondence between pairs of L1C and MARIDA patches. %Correct matches are shifted by very similar amounts, while the shifts of incorrect ones usually differs significantly from the correct matches. 
%Discarding the outliers was found to be beneficial.


$\mu$ and $\sigma$ are respectively the mean and the standard deviation of horizontal or vertical differences, depending on whether horizontal or vertical differences are examined to be discarded. If a horizontal difference is discarded, its corresponding vertical difference is discarded too (and vice-versa). 

Afterward, the mean of both horizontal and vertical shifts is recomputed with the shifts that were not discarded. Let $\bar{s}_h$ be the mean horizontal shift and $\bar{s}_v$ the mean vertical shift.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{images/3_Methods/shifts.png}
    \caption{Suppose the points with the same color in the two different images are matching keypoints (green and red points). The horizontal shifts of the green and red keypoints are respectively $s1_h$ and $s2_h$, while the vertical shifts are $s1_v$ and $s2_v$. In this ideal case, the keypoints match perfectly and so $s1_h = s2_h$ and $s1_v = s2_v$.}
    \label{Figure:shifts_example}
\end{figure}

In step \second, the shifts $\bar{s}_h$ and $\bar{s}_v$ are applied to the MARIDA patch center's coordinates (the original center's coordinates). Figure \ref{Figure:shift_centers} shows an illustration of step \second, where Image B is an image that contains Image A (as the L1C patch contains the MARIDA one). The coordinates of the center of Image A inside Image B (light blue point) are found by applying the computed $\bar{s}_h$ and $\bar{s}_v$ to the original center coordinates of Image A (orange point).

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{images/3_Methods/shift_center.png}
    \caption{Illustration of step \second: applications of the shifts to the center coordinates.}
    \label{Figure:shift_centers}
\end{figure}

Lastly, in step \third, the larger L1C patch (all of its 13 bands) is cropped by setting the shifted coordinates of the center of the MARIDA patch as the new center, and dimensions equal to the MARIDA patch's dimensions. Figure \ref{Figure:crop_final_step} shows an illustration of this step. The red box represents the cropping area, its content is equal to Image A, and its dimensions are equal to the width and height of Image A. Figure \ref{Figure:marida_l1c_cropped} shows an example of the final result of a MARIDA patch and its cropped corresponding L1C patch.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.85\textwidth]{images/3_Methods/crop.png}
    \caption{Illustration of step \third: cropping of a smaller image from a larger one.}
    \label{Figure:crop_final_step}
\end{figure}


\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{images/3_Methods/L1C/after_keypoints_and_cropping.pdf}
    \caption{Comparison of band B1 of a MARIDA patch and its cropped corresponding L1C patch.}
    \label{Figure:marida_l1c_cropped}
\end{figure}




\subsubsection{Missing tiles and patches}

Some tiles were not found when downloading data from the Copernicus Open Access Hub in \ref{subsubsec:image-retr}. The tile names that were missing are \textit{S2\_12-1-17\_16PCC}, \textit{S2\_21-2-17\_16PCC}, and \textit{S2\_12-1-17\_16PEC}. The first two tiles respectively contains 28 and 25 patches of the training set of the MARIDA dataset, while the latter tile contains 40 patches of the validation set of the MARIDA dataset. Moreover, two L1C patches that were originally from the validation set of the MARIDA dataset (\textit{S2\_18-9-20\_16PCC\_47}, and \textit{S2\_18-9-20\_16PCC\_48}) were excluded because their pixels were all equal to zero. The presence of only zero pixels could be due to the fact of not finding any matching keypoints for these two patches. Thus, a total of 95 patches are missing in the L1C dataset compared to the original MARIDA dataset.  

%missing tiles (from Cop Hub):

%S2_12-1-17_16PCC
%S2_12-1-17_16PEC
%S2_21-2-17_16PCC

%missing tiles names and corresponding patches when collecting L1C data:
%S2_12-1-17_16PCC => 28 patches -> were in the train split
%S2_12-1-17_16PEC => 40 patches -> were in the val split
%S2_21-2-17_16PCC => 25 patches -> were in the train split
%=> a total of 93 missing patches

%(I checked this and indeed 93 patches are missing in l1c_data)

%I also excluded these 2 patches:
%'data/l1c_data/tif_final/S2_18-9-20_16PCC_47.tif'
%'data/l1c_data/tif_final/S2_18-9-20_16PCC_48.tif'
%-> these 2 were both in the val set

%because their values were all = 0.
%=> a total of 95 missing patches.


%patches for which I found 2 tiles on Cop Hub, which I included them both -> make sure that they correspond to MARIDA images them (when generating the L1C dataset before training):
%S2_22-12-20_18QYF
%S2_20-8-18_16PCC


==> 4_ResultsAblation_study_lr_decay.tex <==
\subsection{Ablation Study - Learning Rate Decay in Fully-Supervised Models}
\label{subsubsec:results_fully-sup-baseline}

Table \ref{table:exp-lr-decay-vs-no-lr-decay} compares fully-supervised models with and without the application of learning rate decay at the \nth{40} epoch. Three distinct percentages of labeled training data were considered. 


The fully-supervised models that do not decay the learning rate at the \nth{40} epoch have higher \gls{mIoU} scores across all examined subsets of training data. Specifically, when utilizing 10\%, 50\%, and 80\% of the labeled data, the \gls{mIoU} score shows an increase of 27\%, 8\%, and 6\% respectively.






\begin{table}[H]
\caption{Test \gls{mIoU} scores of fully-supervised models trained with and without learning rate decay with three different percentages of the full training set. The tested learning rate decay multiplies the learning rate by $0.1$ at the \nth{40} epoch.}
\label{table:exp-lr-decay-vs-no-lr-decay}
\centering
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{llll}
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{3}{c}{Labeled data (\%)}                 \\ 
    \cmidrule{2-4} 
                            & \multicolumn{1}{l}{10} & \multicolumn{1}{l}{50} & 80 \\ 
    \midrule
    Lr decay - epoch 40     & \multicolumn{1}{l}{0.41}   & \multicolumn{1}{l}{0.78}   &  0.85  \\
    No lr decay             & \multicolumn{1}{l}{\textbf{0.68}}   & \multicolumn{1}{l}{\textbf{0.86}}   & \textbf{0.91}   \\ 
    \bottomrule
\end{tabular}
\end{table}


Figures \ref{Figure:lr_decay_vs_without_exp_10}, \ref{Figure:lr_decay_vs_without_exp_50}, and \ref{Figure:lr_decay_vs_without_exp_80} respectively show the validation \gls{mIoU} scores across the training steps with 10\%, 50\%, and 80\% of labeled training data. 
The x-axis in all three figures indicates the count of training steps.

As observed in Figures  \ref{Figure:lr_decay_vs_without_exp_10}, \ref{Figure:lr_decay_vs_without_exp_50}, and \ref{Figure:lr_decay_vs_without_exp_80}, the model trained with learning rate decay has a validation \gls{mIoU} that is consistently lower than the model trained without learning rate decay. Moreover, the \gls{mIoU} trends of the fully-supervised models with learning rate decay significantly plateau after a certain number of training steps. In particular, the 10\%, 50\%, and 80\% cases plateau approximately after the \nth{37} (\nth{484}), \nth{78} (\nth{5397}), and \nth{83} (\nth{9134}) epoch (step) respectively. Based on these results, we chose to not apply learning rate decay in all of our other experiments.

 




\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{images/4_Results/lr_decay_vs_without/lr_decay_vs_witouth_10.pdf}
    \caption{Validation \gls{mIoU} scores across the training steps with 10\% of labeled data. The y-axis represents the validation \gls{mIoU} scores, while the x-axis represents the number of training steps.}
    \label{Figure:lr_decay_vs_without_exp_10}
\end{figure}



\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{images/4_Results/lr_decay_vs_without/lr_decay_vs_witouth_50.pdf}
    \caption{Validation \gls{mIoU} scores across the training steps with 50\% of labeled data. The y-axis represents the validation \gls{mIoU} scores, while the x-axis represents the number of training steps.}
    \label{Figure:lr_decay_vs_without_exp_50}
\end{figure}



\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{images/4_Results/lr_decay_vs_without/lr_decay_vs_witouth_80.pdf}
    \caption{Validation \gls{mIoU} scores across the training steps with 80\% of labeled data. The y-axis represents the validation \gls{mIoU} scores, while the x-axis represents the number of training steps.}
    \label{Figure:lr_decay_vs_without_exp_80}
\end{figure}




==> 4_ResultsOne_train_set.tex <==
\subsection{Fully- versus Semi-Supervised Learning Models with One Training Set}
\label{subsec:res-fs-vs-ssl-1-train-set}


Table \ref{table:mIoU-fully-vs-ssl_one_train_set} shows 

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[H]
\begin{adjustbox}{width=\columnwidth,center}
\centering
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{l|llllll}
\hline
                 & \multicolumn{6}{c}{Class}                                                                                                                                            \\ \hline
Method           & \multicolumn{1}{l|}{Marine Debris} & \multicolumn{1}{l|}{A/NOM} & \multicolumn{1}{l|}{Ship} & \multicolumn{1}{l|}{Clouds} & \multicolumn{1}{l|}{Marine Water} & mIoU \\ \hline
Fully-Supervised & \multicolumn{1}{l|}{0.66}             & \multicolumn{1}{l|}{0.91}     & \multicolumn{1}{l|}{0.86}    & \multicolumn{1}{l|}{0.99}      & \multicolumn{1}{l|}{1.0}            & 0.88    \\ \hline
Semi-Supervised  & \multicolumn{1}{l|}{0.71}             & \multicolumn{1}{l|}{0.94}     & \multicolumn{1}{l|}{0.84}    & \multicolumn{1}{l|}{0.97}      & \multicolumn{1}{l|}{0.99}            & \textbf{0.89}    \\ \hline
\end{tabular}
\end{adjustbox}
\caption{Test IoU and mIoU of classes .... A/NOM is the abbreviation of Algae/Natural Organic Material.}
\label{table:mIoU-fully-vs-ssl_one_train_set}
\end{table}

==> 5_DiscussionAblation_study_lr_decay.tex <==
\subsection{Ablation Study - Learning Rate Decay in Fully-Supervised Models}
\label{subsubsec:disc_fully-sup-baseline}

This experiment compares the performance of fully-supervised models trained with and without learning rate decay applied at the \nth{40} epoch. The decay was performed by multiplying the learning rate by $0.1$. The comparison of a pair of models (with versus without learning rate decay) is performed by using three different percentages of labeled data: 10\% (low), 50\% (medium), and 80\% (high).


As indicated in Table \ref{table:exp-lr-decay-vs-no-lr-decay}, the fully-supervised models that did not utilize learning rate decay outperformed those that did. This was consistent across all three distinct percentages of labeled training data.

Figures  \ref{Figure:lr_decay_vs_without_exp_10}, \ref{Figure:lr_decay_vs_without_exp_50}, and \ref{Figure:lr_decay_vs_without_exp_80} show that the validation \gls{mIoU} trend of the models trained with learning rate decay at the \nth{40} epoch is consistently lower compared to the models that does not implement learning rate decay. Furthermore, the \gls{mIoU} trends of the fully-supervised models with learning rate decay plateau.

This behaviour is probably due to the fact that applying the decay at \nth{40} epoch prematurely reduces the learning rate. As a result, the steps of the gradient descent become too small to reach a more optimal minimum.


==> 5_DiscussionOne_train_set.tex <==
\subsection{Fully- versus Semi-Supervised Learning Models with One Training Set}
\label{subsec:disc-fs-vs-ssl-1-train-set}

==> lib/kthcolors.tex <==
%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:
% KTH colors for LaTeX documents
%
% Started from kthcolors by:
% Riccardo Sven Risuleo
% 2016-09-06 11:05:40
%
% from https://github.com/KTH-AC/kthcolors
%
% Adapted using the colors from "Graphic Profile Manual KTH" version 180604
% (i.e.. 2018-06-04) 
% see https://intra.kth.se/en/administration/kommunikation/grafiskprofil/kth-s-grafiska-profil-1.844676
% 
% G. Q. Maguire Jr.
% 2021-07-05
%

%\NeedsTexFormat{LaTeX2e}[1994/06/01]
%\ProvidesPackage{kthcolors}[2021/07/85 v3 Latex package with official KTH colors]

\RequirePackage{xcolor}
%% Primary colors
%% As of the new manual, there is only 1 primary color; but with three 
\definecolor{kth-blue}{RGB/cmyk}{25,84,166/0.849,0.494,0,0.349}
\colorlet{kth-blue80}{kth-blue!80!}
\colorlet{kth-blue40}{kth-blue!40!}

% these are no longer used as of 2018-06-04
%\definecolor{kth-red}{RGB/cmyk}{157,16,45/0,0.898,0.713,0.384}
%\definecolor{kth-green}{RGB/cmyk}{98,146,46/0.329,0,0.685,0.427}

%% Secondary colors
\definecolor{kth-lightblue}{RGB/cmyk}{36,160,216/0.833,0.259,0,0.153}
\colorlet{kth-lightblue80}{kth-lightblue!80!}
\colorlet{kth-lightblue40}{kth-lightblue!40!}

%\definecolor{kth-lightred}{RGB/cmyk}{228,54,62/0,0.763,0.728,0.106}
\definecolor{kth-lightred}{RGB}{216,84,151}
\colorlet{kth-lightred80}{kth-lightred!80!}
\colorlet{kth-lightred40}{kth-lightred!40!}

\definecolor{kth-lightgreen}{RGB/cmyk}{176,201,43/0.124,0,0.786,0.212} % olive
\colorlet{kth-lightgreen80}{kth-lightgreen!80!}
\colorlet{kth-lightgreen40}{kth-lightgreen!40!}

% Cool Gray 9C
%\definecolor{kth-coolgray}{RGB}{101,101,108}

% Cool Gray 10 suggested by Martin Krzywinski (see http://mkweb.bcgsc.ca/colorblind) 
\definecolor{kth-coolgray}{RGB}{99,102,106}
\colorlet{kth-coolgray80}{kth-coolgray!80!}
\colorlet{kth-coolgray40}{kth-coolgray!40!}

% Tertiary colors (yet more colors)
% All of these are no longer used
%\definecolor{kth-pink}{RGB/cmyk}{216,84,151/10,0.611,0.301,0.153}
%\definecolor{kth-yellow}{RGB/cmyk}{250,185,25/0,0.26,0.9,0.0196}
%\definecolor{kth-darkgray}{RGB/cmyk}{101,101,108/0.0648,0.0648,0,0.576}
%\definecolor{kth-middlegray}{RGB/cmyk}{189,188,188/0,0.00529,0.00529,0.259}
%\definecolor{kth-lightgray}{RGB/cmyk}{227,229,227/0.00873,0,0.00873,0.102}

%\DeclareOption{gray}{\colorlet{gray}{kth-darkgray}}

% These versions are designed to meet accessability requirements for digital media
% Note that the palette is more limited than for the print version of the colors
\ifdigitaloutput
    % primary color
    \definecolor{kth-blue}{HTML}{1954A6} % Deep sea
    \definecolor{kth-blue80}{HTML}{5E87C0}

    % Secondary colors
    \definecolor{kth-lightblue}{HTML}{2191C4} % Stratosphere
    \definecolor{kth-lightred}{HTML}{D02F80} % Fluorescence
    \definecolor{kth-lightred80}{HTML}{D95599}
    \definecolor{kth-lightgreen}{HTML}{62922E} % Front-lawn
    \definecolor{kth-coolgray}{HTML}{65656C} % Office
    \definecolor{kth-coolgray80}{HTML}{848489}
\fi


